Accuracy and precision of industrial stellar abundances

There has been an incredibly large investment in obtaining high-resolution stellar spectra for determining chemical abundances of stars. This information is crucial to answer fundamental questions in Astronomy by constraining the formation and evolution scenarios of the Milky Way as well as the stars and planets residing in it. We have just entered a new era, in which chemical abundances of FGK-type stars are being produced at industrial scales, where the observations, reduction, and analysis of the data are automatically performed by machines. Here we review the latest human efforts to assess the accuracy and precision of such industrial abundances by providing insights in the steps and uncertainties associated with the process of determining stellar abundances. To do so, we highlight key issues in the process of spectral analysis for abundance determination, with special effort in disentangling sources of uncertainties. We also provide a description of current and forthcoming spectroscopic surveys, focusing on their reported abundances and uncertainties. This allows us to identify which elements and spectral lines are best and why. Finally, we make a brief selection of main scientific questions the community is aiming to answer with abundances.

==> Old_surveys.tex <==
RAVE 

%As stated by the authors themselves ``The drawback of this method is that the EWs of the lines are computed by neglecting the opacity of the neighbouring lines'' \citep{2011AJ....142..193B}. %Boeche. 
%Several tests were performed to assess the performances of that procedure and to determine the accuracy of the abundances. 
%In order to assess the performances of the procedure and to determine the accuracy of abundances, the pipeline was run on synthetic spectra with different levels of added noise. The pipeline was also applied considering errors in atmospheric parameters. Observations of stars with abundances known to high accuracy were performed for comparison with the results of the pipeline. Those validation stars were chosen from two large catalogues that were available at that time \citep[][consisting of approx 750 and 200 stars, respectively]{2005A&A...438..139S, 2010ApJ...721L..92R}. Internal errors were evaluated from repeat observations of the same stars. The combination of these different tests showed the typical accuracy to be 0.2~dex depending on S/N and atmospheric parameters. 


%The chemical pipeline was further improved for DR4 \citep{2013AJ....146..134K} with better atmospheric parameters in input, corrections for the opacity of the neighbouring lines, improved line profile \uh{how, in what sense?} and continuum re-normalization. An important aspect of the new pipeline was the calibration of metallicities which had a strong impact on the other abundances. A correction depending on gravity was applied to the metallicities obtained by the atmospheric parameter pipeline which uses a combination of a decision-tree algorithm
%\citep[DEGAS, ][]{Bijaoui_2012} and a projection method
%\citep[MATISSE, ][]{2006MNRAS.370..141R}. The calibration was based on RAVE observations or RAVE-like spectra of a number of reference dwarf and giant stars taken from different sources. The calibration data sets included stars from two open clusters, IC4651 \citep{2004A&A...424..951P} and M67 \citep{2010A&A...511A..56P}, the extremely metal-poor giant CD $-$38 0245 \citep{2004A&A...416.1117C}, and various stars chosen from \cite{2011ApJ...737....9R}, and PASTEL \citep{2010A&A...515A.111S}. That release has 425\,561 entries but provides abundances of Mg, Al, Si, Ti, Fe and Ni  only for 313\,874 spectra that met specific criteria on \teff, S/N and rotational velocity.  The errors were estimated to range from 0.17~dex for Mg, Al, and Ti to 0.3~dex for Ti and Ni and to be 0.23~dex for Fe. Quality flags allow the users of the catalogue to select the most reliable abundances for 187\,305 spectra. 
 
%For the fifth and latest release including the final RAVE observations \citep{2017AJ....153...75K}, the chemical pipeline was similar to the previous one but the atmospheric parameters improved thanks to a larger sample of calibration stars that became available.  The new  sample was expanded toward the high-metallicity end to better calibrate the tails of the distribution function with stars taken from the catalogues of \cite{2012A&A...542A..48W} and \cite{2013A&A...554A..44A}. \gbs s were also included, observed with RAVE or with RAVE-like spectra derived from the library of \cite{GBS2}. Surface gravities were calibrated using both the asteroseismic \logg\ values of 72 giants from K2 \citep{2017A&A...600A..66V} and the \gbs s. With these improved calibrations the abundance errors were found to be $\sim$0.2~dex for Mg, Al, Si, Ca, Ti, and Fe and 0.25~dex for Ni. \uh{for how many spectra and how many stars?} While the general precisions  have remained  over the data releases, they are believed to be more accurate thanks to the improvement in input parameters needed to derive abundances. 


GES
%Description of spectra (where, when, R, lambda, mag range?)
%Description of chemical pipeline (which elements and linelist)
%Description of prescription for spectral analysis
%Description of pipeline for parameters, specifying the calibration and validation strategies
%Discussion of uncertainty tests for abundances
%summary of number of elements, stars and typical accuracies. 
%Other datasets 



APOGEE
Empirical calibrations of stellar parameters were presented for the first APOGEE data release (SDSS DR10) by \cite{2013AJ....146..133M}. These calibrations were enabled by observations of 559 stars in 20 globular and open clusters supplemented by asteroseismic targets with well determined gravities from the Kepler field. \pj{Here maybe a paragraph of APOCASK}. The performances of ASCAP in DR12 were assessed with members of the benchmark open cluster M67  \citep{2016AJ....151..144G}. The O, Ca, and Fe abundances showed small dispersion (0.03--0.04 dex) and little or no trend
with \teff\ while the Si, Ti, and Mn abundances showed clear trends resulting from systematic ASPCAP errors. \cite{2015AJ....150..148H} applied internal and external empirical calibrations in chemical abundances using as reference a set of 22 globular and open clusters spanning a wide range of
metallicity. The internal calibration was intended to improve the homogeneity of abundances within clusters, while  the external calibration was intended to improve the agreement of the metallicity of metal-poor clusters with previously measured values. Abundances of C, N, O, Na, Mg, Al, Si, S, K, Ca, Ti, V, Mn, Fe, Ni were provided with a precision of 0.05 to 0.09 dex. The accuracy of the abundances was assessed by comparison with other measurements of individual stars including the Sun and Arcturus and was estimated to be 0.1--0.2 dex. SDSS DR14 is described by \cite{2018ApJS..235...42A}, including the first data from APOGEE-II, corresponding to $\sim$260\,000 stars.  In addition to the ASCAP stellar parameters and abundances, {\it The Cannon}  \citep{2015ApJ...808...16N} modified by \cite{2016arXiv160303040C} has also been applied and is provided as part of DR14. \pj{Are they discussed in the last paper of Holtzman, right?}. 


An accurate and self-consistent chemical abundance catalogue for the APOGEE/Kepler sample was delivered by \cite{2016A&A...594A..43H} providing abundances of C, N, O, Mg, Ca, Si, Ti, S, Al, Na, Ni, Mn, Fe, K, P, Cr, Co, Cu, Rb, Yb and V in for the APOCASK stars
derived with the code BACCHUS \citep{2016ascl.soft05004M} where \teff\ and  \logg\ were kept fixed. This dataset is proposed as a a reference set. The code was validated against some \gbs\ (The Sun, Arcturus, and $\mu$ Leo) and open and globular clusters. High precision is achieved by differential abundances with Arcturus. %That work showed the importance of line selection. 
Typical uncertainties have been assessed by repeating the analysis after varying the atmospheric parameters and comparing the different analysis methods employed by BACCHUS. Their determined abundances show small
differences to that of DR12 for many elements, but significant differences regarding Si, S, Ti, and V.

APOGEE is the first ambitious project to collect near IR spectra, opening a new window of spectroscopy and pushing the progress in modelling of spectral lines which for long has been essentially unexplored. 



 In \cite{2018ApJ...853..198N}, {\it The Cannon} has been modified to take into account the varying PSF across the detector of APOGEE. It is applied to 90 members of 7 open clusters, plus $>$1000 field stars in order to evaluate the chemical similarity among field stars and among stars with a common birth origin. An assessment of abundance precision was performed with cross-calibrations where 10\% of the calibration set (5000 giant stars with S/N $>$200 ans ASPCAP parameters) is left apart for comparisons to the reference values while the remaining 90\% is used to construct the model.  Abundances of Fe, C, N, O, Na, Mg, Al, Si, S, K, Ca, Ti, V, Mn, Ni, P, Cr, Co, Cu, Rb  were provided at a precision of 0.02 to 0.12 dex, depending on the element. \pj{Is this dataset public or was just used for the analysis?}

\cite{2018arXiv180709784J} compared stellar parameters and abundances from APOGEE 13 and 14, determined with the ASPCAP pipeline and by {\it The Cannon}, with independent analyses. They selected five studies in the literature with high quality parameters and abundances that had at least 100 stars in common with APOGEE. The comparisons were restricted to stars with calibrated parameters in AOPGEE, so subgiants and giants which are anyway dominating in the survey. For most of the elements (C, Na, Mg, Al, Si, S, Ca, Cr, Mn, Ni) the DR14 ASPCAP analysis have systematic
differences to the comparison samples of less than
0.05 dex (median), and random differences of less than
0.15 dex (standard deviation). Fe, Mg and Ni are the elements which show the best agreement with reference values.


\pj{Taken from common elements section of Ulrike: presicion assessment should be discussed here: }
The accuracy of abundances was evaluated by comparison to independent optical and near-IR spectroscopic analyses of nearby stars and stars in globular clusters reported in the literature. The general conclusion was that the abundances have an accuracy of 0.1--0.2~dex, although abundance differences of up to $\pm$0.4~dex were seen for all elements for a significant number of stars. Differences up to +0.6~dex (APOGEE minus comparison stars) occurred for some stars in globular clusters, and for Na and Mn also for a few of the optically analysed field stars.



\pj{Taken from problematic elements ulrike}

\pj{Here a discussion on difficult elements in IR as done previously for the easy elements}
%Concerning the IR region, \citet{2015AJ....149..153M} % Meszaros et al.
determined abundances for nine elements in ten globular clusters from APOGEE DR10 spectra (using the DR12 line list described in \citealt{2015ApJS..221...24S}).
A comparison of their results with literature values showed a general agreement within $\pm$0.2~dex, except for Al, Ca, and Ti for stars with low abundances of these elements relative to Fe, for which the APOGEE analysis gave up to 0.8~dex higher abundances than the comparison sources.


 
% cf. Heiter et al. Section 6.1

An alternative way for investigating the issue at hand can be found in 
\citet{GBS4}, % Jofre et al. (2015) - GBS Paper IV
who derived abundances of $\alpha$-capture and iron-peak elements for the \gbs\ using several methods. The abundances were derived both in an absolute sense and differentially (line-by-line) with respect to reference stars with similar atmospheric parameters.
Problematic elements may be identified as those for which the LLS is significantly lower for the differential abundances than for absolute abundances. At solar metallicity this was the case for Sc, Mn. %, Mg (dwarfs only), and Ca (giants only).
%
The element-specific reasons for the difference in the LLS according to that work were effects of hyperfine structure for Mn lines, which had not been modelled by all of the methods, and large uncertainties in atomic data for Sc lines. %For Mg and Ca no clear explanation could be found. The Ca abundances in giants may be particularly susceptible to issues of line selection, as only one third of the lines available for dwarfs could be used for the giants.
%A large variation in line selection between different groups of stars was also seen for Ti and Cr (about 50 and 70 percent of lines available for solar-metallicity dwarfs were used for giants, respectively), with seemingly smaller effects on the LLS in abundances.

%\uh{The following assumes that golden lines are introduced earlier in the review (Sect.~\ref{sect:line_selection}).}
%The results were inconclusive for metal-poor stars.
%However, 
The most problematic elements for this metal-poor seem to be V and Co, which did not have any golden lines (as defined in \citealt{GBS4}) out of $\sim$30 and $\sim$20 lines available in the line list, and for which no abundance could be determined for some of the metal-poor stars.
%Keeping the focus on metal-poor stars, we 
Let us take as an example the work by 
\citet{2016MNRAS.460..884H} % Howes et al. (2016) - EMBLA
done within the EMBLA survey of the Milky Way bulge.
Abundances of 19 elements were derived from high-resolution spectra using EWs. The spectra covered a larger wavelength range (333--941~nm for most stars) and so the list of spectral lines and atomic data had partial overlap with the GES one. In this work the species with the highest uncertainties in abundance ($\gtrsim$0.2~dex) were \nai, \cri, \mni, \coi, \nii, and \srii\ 
(V abundances were not derived).  Because in metal-poor stars lines are weaker, effects of hyperfine structure on Mn and Co lines were assessed to be negligible.

The GES line list contains an assessment of the blending properties of over 1300 lines of 35 elements, based on visual inspection of observed and synthesised line profiles for the Sun and Arcturus. An investigation of this characteristic together with the quality of oscillator strengths allows one to identify the most problematic elements in the optical wavelength region (Heiter et al., in preparation).
% cf. Heiter et al. Section 6.2
The most problematic element turns out to be Sr, for which the ten available \sri\ lines all are very weak, blended, and have uncertain atomic data.
% The same applies to V~I and Y~I, but for those elements abundant high-quality lines of the other ionisation stage are available.
The situation is also problematic for the species \ali, \si, and \crii,
%Al~I, S~I, and Cr~II,
for which lines suitable for abundance analysis are available, but they all have uncertain atomic data. 
Somewhat better but still unsatisfactory cases are represented by the species  \nai, \mgi, \sii, \caii, and \nii,
%Na~I, Mg~I, Si~I, Ca~II, and Ni~I,
for which numerous unblended lines are available, but the majority of these are in need of improved atomic data.
For \ali\ and \sii\ this indicates that the abundances derived in optical spectra might be affected by significant systematic uncertainties, despite the high precisions mentioned in Sect.~\ref{sect:common_elements}.

\pj{Discuss non-LTE effects, and very rare elements in periodic table as well as in Hypatia. Is it because few lines available, blended?}


\pj{Discuss what should happen to fill the rest of the periodic table? R-process not included at all in industrial surveys, why?}


OLD TOOLs: into table tools


%\subsubsection{Model atmospheres, radiative transfer calculators, grids of synthetic spectra}
%Model atmospheres in 1D that are used by the works discussed in this review are MARCS \citep{2008A&A...486..951G} and  ATLAS9 \citep{2003IAUS..210P.A20C}. For public 3D model atmospheres we refer to the {\tt STAGGER} \citep{2013A&A...557A..26M} grid and CO5BOLD \pj{is it public? what is the reference, is there another?}.  Regarding radiative transfer codes, those employed for the results discussed in this review are Turbospectrum \citep{1992A&A...256..551P}, MOOG \citep{1973PhDT.......180S}, SYNTHE \citep{1993sssp.book.....K}, SPECTRUM \citep{1994AJ....107..742G} \pj{One non-LTE code?}. 


%\subsubsection{Atomic and molecular data}
%A popular source for transition data comes from the Vienna Atomic Line Database \citep[VALD][]{2015PhyS...90e4005R}.  It is one of the largest databases as its collection includes all sources available, regardless of their accuracy and current extensions include molecular data. Other equally source of atomic data comes from the National Institute of Standards and Technology (NIST)' Atomic Spectroscopy Data Center \pj{Is there a reference paper?}.  Like VALD, this database contains references to publications on atomic transition probabilities.  The series of works Sneden, Lawler, Wood and colleagues also have compiled a large line list which can be downloaded from a website\footnote{\url{https://www.as.utexas.edu/~chris/lab.html}}. The websites of R. Kurucz\footnote{\url{http://kurucz.harvard.edu/linelists/}} provide extensive information about molecular and atomic transitions, among which many are ingested in VALD or NIST but can be used independently. 
%Molecular linelists are extensively developed by \cite{2014A&A...571A..47M} and can be obtained upon request. The ExoMol database \citep{2016JMoSp.327...73T} provides further molecular transitions for astronomers which are valid over extended temperatures ranges, focused at the cool end of the spectrum. The Belgian Repository of Fundamental Atomic Data and Stellar Spectra \citep[BRASS,][]{2018Galax...6...78L} is aiming at centralising all this information in one single website.  

%\subsubsection{Grids of synthetic spectra} 
%Atmosphere models, radiative transfer codes and line list allow to compute synthetic spectra. Public grids of spectra at a large parameter space are AMBRE \citep{2012A&A...544A.126D}, which is focused on high resolution optical spectra;  STAGGER \citep{2018A&A...611A..11C}, which is focused on the Gaia RVS range (see Sect.~\ref{sect:surveys}). \cite{2018A&A...615A.139A} provide a grid of synthetic spectra around the Balmer lines computed with 3D-non-LTE.  \cite{2012AJ....144..120M} provide one for infrared spectra dedicated to APOGEE. 

%\subsubsection{Tools to prepare and analyse spectra} Many codes that determine abundances from spectra by performing fitting to line profiles or measuring EWs also have the tools to correct by radial velocities and normalise.  Spectroscopy Made Easy \citep[\tt{SME}]{2017A&A...597A..16P} determines abundances by performing a fitting of on-the-fly synthetic spectra to observations.  Among the wrapper codes, one that has attracted attention is {\tt iSpec} \citep{2014A&A...569A.111B}, which perform spectral synthesis using the different radiative transfer and model atmospheres listed above, allowing for systematic comparison of methods and input data.
%BACCHUS \citep{2016ascl.soft05004M} \pj{public?}. C. Allende Prieto has developed FERRE\footnote{\url{http://leda.as.utexas.edu/ferre/}}, which matches physical models to observed data to determine stellar parameters. GALA automatically derives atmospheric parameters and abundances for individual species using EWs of metallic lines. \citep{2013ApJ...766...78M}. Codes focused to automatic determinations of EWs are DAOSPEC \citep{2008PASP..120.1332S} and its wrapper DOOp \citep{2014A&A...562A..10C}.  ARES \citep{2015A&A...577A..67S} is widely used in particular to characterise planet host stars. \pj{Marcelo compares them}.  

%\pj{Other data-driven codes SICK, The Cannon,  Ting page, latest AAN of Bovy}. 


%\subsubsection{non-LTE corrections and other empirical calibrations}
%the pages of inspect. Photometric calibrations for teff, calibrations for vmic. 





==> differential_analysis.tex <==




\subsection{metal-poor stars, galactic evolution, tagging} 

\begin{itemize}

\item A DIFFERENTIAL ABUNDANCE ANALYSIS OF VERY METAL-POOR STARS 
%OMalley_2017ApJ.838.90O.pdf

\item First high-precision differential abundance analysis of extremely metal-poor stars
%Reggiani_2016A&A...586A..67R.pdf

\item possible dependence of the Tc trend on stellar Galactocentric distances, Rmean 
%Adibeykyan 2016A&A...592A..87A.pdf

\item Two distinct halo populations in the solar neighborhood- Evidence from stellar abundance 
ratios and kinematics 
%Nissen_2010A&A_511L_10N.pdf

\item High-precision abundances of elements in Kepler LEGACY stars Verification of trends 
with stellar age 
%Nissen_2017arXiv171003544N.pdf

\item Nucleosynthetic history of elements in the Galactic disk [X/Fe]–age relations from 
high-precision spectroscopy 
%Spina_2016A&A...593A.125S.pdf
\end{itemize}


==> sect_common_elements_v1.tex <==



\begin{figure}
\includegraphics[scale=0.45]{Figures/JofreFig8.pdf}
\caption{Periodic table annotated with the surveys for which lines of a given element can be detected. Elements in squares are included in Hypatia, but are not planned to be studied in spectroscopic surveys.} 
\label{fig:periodic_table_surveys}
\end{figure}


Widely measured elements can be identified in the histogram of Figure~\ref{4.hypatia} as those that have more than $\sim$4000 measurements, and are covered by at least all surveys with high resolution and large wavelength coverage (GALAH, GES, and APOGEE, see Figure~\ref{fig:periodic_table_surveys}). 
These are C, O, Na, Mg, Al, Si, Ca, Ti, V, Cr, Mn, Fe, Co, and Ni. Cu and Nd are common elements targeted by surveys but not as common as the others in Hypatia.
%The line list papers of GES and APOGEE \citep[Heiter et al, in prep][respectively]{2015ApJS..221...24S} %Shetrone
%are good resources to understand why this is the case. 
% Shetrone et al. do not discuss Cu or Nd.

To evaluate the precision of abundances for these common elements, let us take as an example the abundances published by GES to illustrate the situation in the optical wavelength region. We choose GES because of its unique strategy of combining several results using different methods based on a common list of atomic data with special effort in flagging ``good" and ``bad" lines (see Sect.~\ref{sect:GES} and \citealt{heiter-linelist}). % GES-Linelists manuscript (18 Feb. 2018)
This allows one to assess the method-to-method or line-to-line dispersion (MMD or LLD, respectively) for different species.
The precision of the abundances evaluated using the MMD was found to be highest ($<0.15$ to $0.2$~dex) for the species
%\nai, \mgi, \ali, \sii, \cai, \caii, \scii, \tii, \fei, \cri, and \nii\ (???)
\nai, \mgi, \ali, \sii, \cai, \scii, \tii, \vi, \fei, \zri, \moi, and \baii\
\citep[p.~23]{2014A&A...570A.122S}. % Smiljanic
The elements with precise abundances in common among all setups are \ali, \sii, and \cai.
In the IR, abundances more precise than 0.05~dex in APOGEE DR14 \citep{2018arXiv180709773H} are those of C, O, Mg, Al, Si, Ca, Ti, Cr, Mn, Fe, and Ni.
In summary, popular elements in spectroscopic surveys in the optical and IR that are also precise are Mg, Al, Si, Ca, Ti, and Fe.  These elements all have agreements and biases between optical and IR surveys within the uncertainties \citep{2018arXiv180709784J}. %Jonsson

To discuss these popular elements in more detail, we concentrate on the works of \cite{GBS4} and \citet{heiter-linelist} for the situation in GES, of \cite{2016A&A...594A..43H} %Hawkins 
for the situation in APOGEE, and of \cite{2018arXiv180709784J} for the comparison between the optical and IR. We exclude Fe from this description as being the element with the largest number of lines available in FGK-star spectra, which forms the basis for the metallicity parameter. 
\begin{itemize}
\item {\bf Magnesium} In the GES range, twelve \mgi\ lines are included. Among them, $\lambda 6318$ and $\lambda 6319$\AA\ have accurate atomic data, and are good lines for a variety of stars and methods. In APOGEE there are 14 \mgi\ lines, among which six are suitable for a large variety of stars. Non-LTE corrections have been determined in the optical by \cite{2015A&A...579A..53O},  and in the IR by \cite{2017ApJ...835...90Z} and \cite{2017ApJ...847...15B}.
\item {\bf Aluminum} No reliable experimental transition probability data exist for the five \ali\ lines of GES.
However, none of them is considered heavily blended, possibly explaining the good precision (MMD) achieved despite the lack of reliable laboratory data.
In APOGEE, three \ali\ lines are present, although one ($\lambda 16763$\AA) seems to be more robust for different types of stars. Non-LTE studies of optical and IR lines have been performed by \cite{2017A&A...607A..75N}.  
\item {\bf Silicon} Among the 45 \sii\ lines visible in GES spectra, only three ($\lambda$5690, $\lambda$5701, and $\lambda$5949\AA) have good atomic data and are blend-free in dwarfs and giants. The partially blended line at $\lambda$5708\AA\ with good atomic data is strong enough to be measured in metal-poor stars. APOGEE has 17 \sii\ features, among which five ($\lambda$15377, $\lambda$15888, $\lambda$16216, $\lambda$16681, and $\lambda$16828\AA) are good lines to be used for a variety of stars. Improved modelling for \sii\ lines has been done by \cite{2012ApJ...755...36S} and \cite{2016ApJ...833..137Z} for optical and IR lines. Non-LTE corrections in the optical are provided for the \gbs s by \cite{GBS4}.
\item {\bf Calcium} The GES has 31 \cai\ and eight \caii\ lines detectable, among which twelve and two have reliable laboratory data, respectively. The lines are highly sensitive to stellar parameters and therefore, only one ($\lambda5867$\AA) can be used to derive abundances for a large variety of spectral types (excluding metal-poor stars). In APOGEE, four lines are visible, but only three ($\lambda$16150, $\lambda$16157, and $\lambda$16197\AA) can be used for a wider range in stellar parameters.  Non-LTE corrections in the optical are provided for the \gbs s by \cite{GBS4}. In the IR calculations are needed. 
\item {\bf Titanium} After \fei, \tii\ is the element with the most numerous absorption features, including 105 in GES spectra, among which 23 have good atomic data and are largely blend-free. Three lines ($\lambda$5689, $\lambda$5702, and $\lambda$6091\AA) can be used for elemental abundances in a large variety of stars. In APOGEE nine Ti lines are detected (but see Sect.~\ref{sect:line_selection} for a discussion on their applicability). Non-LTE effects have been studied by \cite{2011MNRAS.413.2184B} for optical lines.  In the IR calculations are needed. 
%\item {\bf Chromium} 64 \cri\ and 24 \crii\ lines exist in the GES spectra, but only 9 \cri\ lines and no \crii\ line have reliable atomic data and are free of blends. The lines $\lambda$5272 and $\lambda$5287\AA\ can be used to analysed a large variety of spectra.  In APOGEE, 8 regions can be used to determine Cr abundances, but \cite{2016A&A...594A..43H} consider only one line ($\lambda 15680$\AA) due to the large blends with telluric features affecting many of the regions. NLTE effects in the optical have been studied by \cite{2010A&A...522A...9B}. In IR calculations are needed. 
%\item {\bf Nickel} There are numerous Ni lines with accurate atomic data which are free of blends, explaining why this element is precise in optical studies in general. Among all the lines, 3 \nii\ ($\lambda$5846, $\lambda$6176 and $\lambda$6327\AA) are good abundance diagnostics for a large variety of stars \citep{GBS4}. In the IR, Ni abundances are measured from 30 regions, several of them with strong and clean lines, explaining the accurate Ni abundances obtained in APOGEE. To our knowledge, no NLTE corrections are publicly available for optical or IR \nii\ lines. 
\end{itemize}

Common elemental abundances which can be precisely measured from IR spectra, but not from optical spectra, are C, O, and Mn. C and O abundances can be derived from molecular features, while few clean Mn lines are suitable. In the optical the situation is more complicated,
% C and molecules are very strong and (???)
as there is only one \ci\ and one [\oi] line which have good atomic data and are free of blends. The \ci\ line is very weak and [\oi] lies in telluric regions. The O triplet at 7770\AA\ is popular, and included in GALAH, but is subject to strong non-LTE effects \citep{2016MNRAS.455.3735A}. For Mn, although many lines are detected in the optical, they are subject to strong HFS, affecting resulting abundances by up to 0.6~dex if HFS is not properly taken into account \citep{GBS6}. 
Sodium is derived with high precision from optical spectra, but has more problems in the IR. There are three \nai\ lines that are considered largely clean in the optical. Although they are subject to HFS, it seems the effect is small, since the LLD and MMD for the abundances are small \citep{2014A&A...570A.122S}. In the IR, the two absorption features are in most cases too weak or blended. Non-LTE effects for \nai\ can be very strong \citep{2011A&A...528A.103L}. Finally, V and Co are elements which are common but more uncertain than the other elements, being subject to HFS. Although V and Co lines are very numerous in the optical, they can be quite weak. They become scarce and too weak in the IR or for metal-poor stars. V and Co abundances are normally derived from blue lines for metal-poor stars \citep{2016ApJ...817...53S}. 



==> sect_complicated_elements.tex <==
The fact that our periodic table in Fig.~\ref{fig:periodic_table_surveys} has most cells unmarked means that, for most of the elements, it is either very challenging or impossible to detect and model lines for typical spectra of FGK-type stars in order to obtain accurate abundances. From Fig.~\ref{fig:periodic_table_surveys}, the elements that are potentially detected in less than two surveys correspond to Li, P, S, K, Sc, Zn, Ge, Rb, Sr, Y, Zr, Nb, Mo, Ru, Ba, La, Ce, Pr, Nd, Sm, Eu, Gd, Dy, and Yb. Most of the abundances provided by surveys for these elements are so uncertain that they are not released publicly. We base our discussion on the information reported by \citet[the GES line list]{heiter-linelist}, \citet[Hypatia]{2014AJ....148...54H}, and \citet[GES-UVES]{2014A&A...570A.122S} for the situation in the optical, and on \cite{2018arXiv180709784J} and \cite{2016A&A...594A..43H} for the situation in the IR.  

In Hypatia, Sc, Zn, Y, and Ba have abundances reported for more than half of the stars (see Fig.~\ref{4.hypatia}). They are popular because they present good clean lines, although very few, and only in the optical. We note, however, that Sc, Zn, and Y have a large MMD in GES. It remains to be seen whether LAMOST-like spectra would present signatures of such elements, provided that data-driven methods were trained on optical spectra. Li, S, Sr, Zr, La, Ce, Nd, Sm, and Eu are reported in Hypatia for less than half of the sample but more than 1000 stars. As in the previous case, these elements present few clean lines only, except for S, Ce, and Nd. S presents several clean features in the IR, making it a precise element in APOGEE, but in the optical this element is more uncertain, with one clean line with good laboratory data only. We include Ce and Nd in this discussion despite being marked by more than two surveys in Fig.~\ref{fig:periodic_table_surveys}. This is because new identifications of \ceii\ and \ndii\ lines in APOGEE spectra have been reported by \cite{2017ApJ...844..145C} and \cite{2016ApJ...833...81H}. In the optical, twelve \ceii\ lines are detected, among which two are free of blends and have good atomic data and can be used for reliable abundance determination. Over fifty optical \ndii\ lines are detected, however, they are subject to hyperfine and isotope splitting, and most of them are very blended.
% \pj{make short note on Li and Eu?}

Elemental abundances that are reported in Hypatia for less than 1000 stars are P, K, Nb, Mo, Ru, Gd, Dy, and Yb. Phosphorus presents three lines in the IR, but they are blended and very weak. The 21 stars with P abundances in Hypatia come from the analysis of IR lines or from UV lines for metal-poor stars. Potassium can be detected in visual spectra, but in a region that is very contaminated with telluric absorption \citep{2017A&A...600A.104M}. % Mucciarelli, Merle \& Bellazzini
There are two K lines in the IR that are slightly blended with CN molecules, but otherwise have good strength for abundance determination for large samples of stars. Since Nb, Gd, and Dy are included in the GES line list, we have marked them in Fig.~\ref{fig:periodic_table_surveys}. However, the nine weak \nbi\ lines are heavily blended. Gd and Dy have one identified line each in GES spectra, but both are very weak and blended in FGK-type stars. The two suitable optical Mo lines are too weak in dwarfs to be useful and Ru has so far only one good line which is partially blended. Although Ru lines are subject to HFS and isotope splitting, because the line is weak these effects are expected to be negligible. While not included in GALAH DR2, these Mo and Ru lines fall within its wavelength coverage and may be included in future data releases \citep{2018MNRAS.478.4513B}. %Buder 

Other elements which can potentially be analysed in optical and IR spectra are rubidium and ytterbium. The \rbi\ line at $\lambda$7800\AA\ has been analysed by \cite{2014AJ....147..136R} %Roederer 
to provide abundances for metal-poor stars and is included in the GALAH spectra. The IR \rbi\ $\lambda$15290\AA\ line is very weak and heavily blended, presenting a challenge for most of the stars observed by APOGEE. In the optical there is an \ybii\ line at $\lambda$3694\AA\ which can be used for analysing metal-poor stars \citep{2014AJ....147..136R}, %Roederer
but it becomes too blended for more metal-rich stars. In the IR, a weak and blended \ybii\ line at $\lambda$16498\AA\ has been identified and could be included in future data releases of APOGEE, provided the syntheses around the blends are accurate. Finally, Ge has the potential to be detected in IR spectra as well. The \gei\ line at $\lambda$16760\AA\ is heavily blended with an \fei\ line at the resolution of APOGEE, but could be resolved at higher resolution.

We finish this section discussing the elements for which abundances are included in Hypatia, but which have no record of detection in spectroscopic surveys. These elements correspond to Be, Pd, Ag, Tb, Er, Tm, Hf, Pb, and Th, and are enclosed with a magenta square in Fig.~\ref{fig:periodic_table_surveys}. Their abundances have been reported in the literature from spectral analyses of FGK-type stars, but mainly from a few lines detected towards the blue end of the visual spectrum \citep{2014AJ....147..136R}. Thus, if nucleosynthesis channels like the rapid neutron-capture process are to be explored in future spectroscopic surveys, it is important to extend the wavelength coverage towards the blue side of the spectrum (see \citealt{2015AN....336..665H} for a discussion for 4MOST). 



==> table_errors.tex <==
\begin{table}[h]
\hspace{-4cm}
\caption{Methods to assess error budget in abundance determination}
\label{tab:errors}
\begin{tabular}{@{}lcccccccc@{}}
\hline
Catalogue & spectra  & lines & modelling &  params & trends & methods & external &  precision \\
\hline
Independent \\
RAVE & repeat &  \\
GES & repeat & \\
GALAH & \\
APOGEE & clusters & \\ 
GBS  & instruments & $\sigma$ & Ion/NLTE & errors & -- & $\sigma$ & Hypatia & differential\\
APOKASC \\
1111 GTO & -- & $\sigma/\sqrt{\mathrm{N}}$ & Ion &  errors & \xfe -\teff & -- & literature & -- \\
SPOCS & repeat & -- & -- & $\sigma\sqrt{\mathrm{\#input}}$ & \xfe -\teff & -- & literature & -- \\
Bensby \\
AMBRE & instruments & \\
\hline
\end{tabular}
\begin{tabnote}
$\sigma$: Standard deviation; N: Number of lines; Ion: Ionisation balance; NLTE: line-by-line corrections when possible;  Catalogue references: GBS: \cite{GBS4}.
\end{tabnote}
\end{table}
%Calibration & 1 & 1 & 1 & 1 & 1 &  & \\
%Survey &  2 & 2 & & 2 & & 2  \\
%High precision & 6 & & 6 &6 & &  \\
%Independent & 3,5& 3,5  & 3 & 3 & 3 &  & 3,5 \\
%\hline
%\end{tabular}
%\begin{tabnote}
%1: \cite{GBS4}; 2: \cite{2014A&A...570A.122S}; 3: \cite{2014AJ....147..136R}; 4: \cite{2017A&A...600A..22M}; 5: \cite{2017MNRAS.470.4363C}; 6: \cite{2016A&A...591A..34A}.
%\end{tabnote}
%\end{table}

==> table_params.tex <==
\begin{table}[h]
\tabcolsep7.5pt
\caption{Methods to determine stellar parameters that are typically employed in automatic abundance pipelines or in the analysis of calibration samples, and their associated uncertainties in abundances.}
\label{tab:params}
\hspace{-2cm}
\begin{tabular}{@{}lcccc@{}}
\hline
Method & Input & Advantage &Disadvantage & Uncertainty \\
\hline\\
&&EFFECTIVE TEMPERATURE&&\\
{\bf IRFM} & photometry, extinction, bolometric flux & available for most stars &difficult in extincted regions.&100~K\\

{\bf Excitation balance} & neutral Fe lines & many clean lines available&non-LTE effects& 60~K\\

{\bf Balmer profiles} & H lines &strong lines & modelling dependency&\\

{\bf Interferometry} &angular diameter, parallax, bolometric flux & independent of spectroscopy &possible for nearby stars only & 50~K \\
\hline\\

&&SURFACE GRAVITY&& \\
{\bf Parallax} & parallax, bolometric magnitude, \teff, mass &independent of spectroscopy &mass dependency & 0.1 dex\\

{\bf Ionisation balance} &neutral and ionised Fe lines & \pj{Advantage?} & difficult to have enough lines & 0.1 dex\\

{\bf Wings of strong lines} & \mgi b, Ca triplets &strong lines &dependency rather weak& \\
{\bf Asteroseismology} & large cadence photometry, \teff & independent of spectroscopy &available for few stars& 0.01~dex\\
\hline\\
&&METALLICITY &&\\

\bf{Iron lines} &Fe lines&many lines available&model dependency& 0.06~dex\\
\bf {Global spectral fitting} &spectrum with some absorption & allows for overall metal content & a suitable grid is needed \\
\hline
%&&MICROTURBULENCE&&\\
%{\bf Weak lines} &neutral lines & many available & not %physical parameter & \\
\hline
\end{tabular}
\begin{tabnote}
$^{\rm a}$Table footnote; $^{\rm b}$second table footnote.
\end{tabnote}
\end{table}
